Efficient Cross-Shard Transaction Execution in Sharded Blockchains

Sharding is a promising blockchain scaling solution. But it currently suffers from high latency and low throughput when it comes to cross-shard transactions, i.e., transactions that require coordination from multiple shards. The root cause of these limitations arise from the use of the classic two-phase commit protocol, which involves locking assets for extended periods of time. This paper presents Rivet, a new paradigm for blockchain sharding that achieves lower latency and higher throughput for cross-shard transactions. Rivet has a single reference shard running consensus, and multiple worker shards maintaining disjoint states and processing a subset of transactions in the system. Rivet obviates the need for consensus within each worker shard, and as a result, tolerates more failures within a shard and lowers communication overhead. We prove the correctness and security of Rivet. We also propose a more realistic framework for evaluating sharded blockchains by creating a benchmark based on real Ethereum transactions. An evaluation of our prototype implementation of Rivet and the baseline two-phase commit, atop 50+ AWS EC2 instances, using our evaluation framework demonstrates the latency and throughput improvements for cross-shard transactions.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

==> sections/implementation.tex <==
\section{Implementation}
\label{sub:implementation}

\noindent
{\bf Existing Implementation.}
Chainspace~\cite{al2017chainspace} built the sharded system from scratch.
It has a python contract environment and java node implementation. It does
not perform rigorous testing. For cross-shard transactions, it only
run transactions with input from multiple shard and output to a single 
shard.

Omniledger~\cite{kokoris2018omniledger} implement from scratch. They don't
evaluate cross-shard transactions.

Dang et al. in~\cite{dang2019towards} implements the sharding on top of
Hyperledger Fabric and Chaincode smart contract platform. They test 
their scheme using KVStore and SmallBank workload. They also vary the
contention using Zipf's distribution. Do not actually evaluate cross-shard
transactions.

Androulaki~\cite{androulaki2018channels} attempts to increase throughput
in Permissionless system. They also end up using two-phase locking. They
don't implement their system.

RapidChain~\cite{zamani2018rapidchain} implements cross-shard transactions.
One good thing about its evaluation is: they consider failures
of nodes. Node inside a shard equivocates with 49\% chance and 49\% of the
node do not participate in the inter-shard communication protocol. They 
claim that around 99\% of the transactions will be cross-shard, as 
transactions are assigned randomly to each shard based on their transaction
id. They don't describe whether their inter-shard transactions are 
conflicting or not. This is not the best design we can have. One should
definitely exploit transaction locality to gain more performance.



\begin{itemize}
    \item Use Quorum which is built on top of Ethereum and currently uses
    Raft consensus protocol. We can plug HotStuff code in it and run it.
\end{itemize}
\begin{itemize}
    \item For better performance, we can use Forkbase as our underlying
    database as it provides efficient roll-back mechanism.
\end{itemize}

==> sections/table.tex <==
% \begin{table}
% \footnotesize
% \centering
%     \begin{tabular}{c|c}
%         \hline 
%         Vertex & Weight \\ 
%         \hline
%         $a_1$ & $1,1,2,4$ \\ 
%         $a_2$ & $1,2,2,4$ \\ 
%         $a_3$ & $1,2,2,4$ \\ 
%         $a_4$ & $3,2,6,9$ \\ 
%         $a_5$ & $1,2,2,4$ \\ 
%         $a_6$ & $3,3,4,11$ \\ 
%         $a_7$ & $2,3,4,8$ \\ 
%         $a_8$ & $2,3,4,4$ \\ 
%         \hline 
%     \end{tabular}
% \end{table}
